Using Hindsight to Anchor Past Knowledge in Continual Learning

In continual learning, the learner faces a stream of data whose distribution changes over time. Modern neural networks are known to suffer under this setting, as they quickly forget previously acquired knowledge. To address such catastrophic forgetting, many continual learning methods implement different types of experience replay, re-learning on past data stored in a small buffer known as episodic memory. In this work, we complement experience replay with a new objective that we call anchoring, where the learner uses bilevel optimization to update its knowledge on the current task, while keeping intact the predictions on some anchor points of past tasks. These anchor points are learned using gradient-based optimization to maximize forgetting, which is approximated by fine-tuning the currently trained model on the episodic memory of past tasks. Experiments on several supervised learning benchmarks for continual learning demonstrate that our approach improves the standard experience replay in terms of both accuracy and forgetting metrics and for various sizes of episodic memories.

==> hal.tex <==
\section{Hinsdight Anchor Learning (\ours{})}
\label{sec:method}

The current state of the art algorithms for continual learning are based on experience replay~\citep{hayes2018memory,riemer2018learning,chaudhry2019er}.
%
These methods learn a predictor $f_\theta$ mapping inputs to logits that, during training, stores a small amount of past observed triplets in an episodic memory $\mathcal{M} = \{(x', y', t')\}$. For a new mini-batch of observations $\mathcal{B} := \{(x, y, t)\}$ from task $t$, the learner samples a mini-batch $\mathcal{B}_\mathcal{M}$ from $\mathcal{M}$ at random, and employ the rule 
$\theta \leftarrow \theta - \alpha \cdot \nabla_\theta \, \ell(\mathcal{B} \cup \mathcal{B}_\mathcal{M})$ to update its parameters, where
\begin{align}
    \ell(\mathcal{A}) = \frac{1}{|\mathcal{A}|} \sum_{(x, y, t) \in \mathcal{A}} \ell(f_\theta(x,t), y)
\end{align}
denotes the average loss across a collection of triplets $\mathcal{A}$. In general, $\mathcal{B}_\mathcal{M}$ is constructed to have the same size as  $\mathcal{B}$, but it can be smaller if the episodic memory $\mathcal{M}$ does not yet contain enough samples.


In the previous, the episodic memory $\mathcal{M}$ reminds the predictor about how to perform at past tasks using only a small amount of data.
%
As such, the behaviour of the predictor outside the data stored in $\mathcal{M}$ is not guaranteed.
%
Furthermore, since $\mathcal{M}$ is usually very small, the performance of the predictor becomes sensitive to the choice of samples stored in the episodic memory.
%
Because of this reason, we propose to further fix the behaviour of the predictor at a collection of carefully constructed \emph{anchor points} $e_{t'}$, one per class per  past task $t'$, at each parameter update.
%\footnote{To ease the exposition, the remaining of the section assumes only one anchor $e_{t'}$ per task $t'$. The extension to one anchor per class per task, as we use in our experiments, is straightforward.}.%; the exact details about the construction of these anchor points will be described soon.

%This setup naturally leads to a meta-learning \citep{finn2017model} formulation. In particular, 
Let us, for now, assume that the anchor points $e_{t'}$ are given. We will see later how to construct these anchor points. To constrain the change of the predictor at these anchor points, we propose a two-step parameter update rule: 
\begin{equation}
\begin{split}
    \tilde{\theta} &\leftarrow \theta - \alpha \cdot \nabla_\theta \, \ell(\mathcal{B} \cup \mathcal{B}_\mathcal{M}), \\
    \theta &\leftarrow \theta - \alpha \cdot \nabla_\theta \biggl( \ell(\mathcal{B} \cup \mathcal{B}_\mathcal{M}) \\
    & + \lambda \cdot \sum_{t' < t} \left(f_\theta(e_{t'}, t') - f_{\tilde{\theta}}(e_{t'}, t')\right)^2 \biggr).
    \label{eq:main_update}
\end{split}
\end{equation}
The first step computes a temporary parameter vector $\tilde{\theta}$ by minimizing the loss at a minibatch from the current task $t$, and the episodic memory of past tasks (this is the usual experience replay parameter update).
%
The second step employs nested optimization to perform the final update of the parameter $\theta$, which trades-off the minimization of ($a$) the loss value at the current minibatch and the episodic memory, as well as ($b$) the change in predictions at the anchor points for all past tasks.
%
%We use L2 over the unnormalized logits as a distance measure in \eqref{eq:main_update}, as we experimentally find it to be superior than cosine similarity or L1 distance.
% 
This two-step nested optimization bears a similarity to gradient-based meta-learning approach~\citep{finn2017model} where we restrict the inner update (the first step) to only a single gradient step. 

Next, let us discuss how to choose the anchor points, $e_{t}$ (one per class per task), such that they can effectively preserve the performance of current task throughout the entire learning experience.
%
To preserve the performance, the anchor points should attempt to minimize the forgetting on the current task as the learner is updated on future tasks.
%
One could achieve this by letting $e_{t}$ be an example from the task $t$ that would undergo maximum forgetting during the entire continual learning experience, including past and future tasks.
%
Then, requiring the predictions to remain invariant at such $e_{t}$, by using~\eqref{eq:main_update}, would minimize forgetting on the current task.
%
Mathematically, the desirable $e_t$ for the label $y_t$ is given by:
\begin{equation} 
    %(e_{t}  \leftarrow \argmax_{x \sim P_t^{y_t}} \, \ell(f_{\theta_T}(x, t), y_t) - \ell(f_{\theta_t}(x, t), y_t),
    e_{t} \leftarrow \argmax_{x \sim P_t(\cdot | y_t)} \, \ell(f_{\theta_T}(x, t), y_t) - \ell(f_{\theta_t}(x, t), y_t),
    \label{eq:ideal_anchor}
\end{equation}
where $\theta_t$ is the parameter vector after training on task $t$ and $\theta_T$ is the final parameter vector after the entire learning experience.
%
Thus, keeping predictions intact on the pair $(e_t, y_t)$ above would effectively preserve the performance of task $t$.
%
However, the idealistic \eqref{eq:ideal_anchor} requires access to ($a$) the entire distribution $P_t(\cdot|y_t)$ to compute the maximization, and ($b$) access to all future distributions $t' > t$ to compute the final parameter vector $\theta_T$. 
%
Both are unrealistic assumptions under the continual learning setup described in Section~\ref{sec:setup}, as the former requires storing the entire dataset of task $t$, and the latter needs access to future tasks. 

To circumvent ($a$), we can recast \eqref{eq:ideal_anchor} as to {\em learn} $e_t$ by initializing it at random and using $k$ gradient ascent updates for a given label $y_t$: 
\begin{equation}
    \begin{split}
    e_t \leftarrow e_t + \alpha \cdot \nabla_{e_t} \biggl( \underbrace{\ell(f_{\theta_T}(e_t, t), y_t) - \ell(f_{\theta_t}(e_t, t), y_t)}_\text{Forgetting loss} \\ 
    - \gamma \underbrace{(\phi(e_t) - \phi_t)^2}_\text{Mean embedding loss} \biggr),
    \end{split}
    \label{eq:anchors_1}
\end{equation}
where we recall that $\phi$ denotes the feature extractor of the predictor, and $\phi_t$ is the neural mean embedding \citep{smola2007hilbert} of all observed examples from task $t$ which regularizes the constructed $e_t$ against the outliers. 
%
Since the feature extractor is updated after experiencing each data point, the mean embeddings $\phi_t$ are computed as running averages.
%
That is, after observing a minibatch $\mathcal{B} = \{(x, y, t)\}$ of task $t$, we update:
\begin{equation}
    \phi_t \leftarrow \beta \cdot \phi_t + (1 - \beta) \frac{1}{|\mathcal{B}|}\sum_{x \in \mathcal{B}} \phi(x),
    \label{eq:mean_embedding}
\end{equation}
where $\phi_t$ is initialized to zero at the beginning of the learning experience.
%
In our experiments, we learn one $e_t$ per class for each task. 
%
We fix the $y_t$ to the corresponding class label, and discard $\phi_t$ after training on task $t$.
%
Learning $e_t$ in this manner circumvents the requirement of storing the entire distribution $P_t$ for the current task $t$.

%While gradient-based optimization bypasses the requirement of storing the entire distribution $P_t$, 
Still, ~\eqref{eq:anchors_1} requires the parameter vector $\theta_T$, to be obtained in the distant future after all learning tasks have been experienced. %for which the learner has no information at the present task $t$.
%
To waive this impossible requirement, we propose to \emph{approximate the future by simulating the past}.
%
That is, instead of measuring the forgetting that would happen after the model is trained at future tasks, we measure the forgetting that happens when the model is fine-tuned at past tasks.
%
In this way, we say that forgetting is estimated in \emph{hindsight}, using past experiences.
%
More concretely, after training on task $t$ and obtaining the parameter vector $\theta_t$, we minimize the loss during one epoch on the episodic memory $\mathcal{M}$ to obtain a temporary parameter vector $\theta_{\mathcal{M}}$, and recast \eqref{eq:anchors_1} as:
%
\vspace{-0.2cm}
\begin{equation}
    \begin{split}
    e_t \leftarrow e_t + \alpha \cdot \nabla_{e_t} \biggl( \ell(f_{\theta_\mathcal{M}}(e_t, t), y_t) - \ell(f_{\theta_t}(e_t, t), y_t) \\ 
    - \gamma (\phi(e_t) - \phi_t)^2 \biggr),
    \end{split}
    \label{eq:anchors_2}
\end{equation}

giving our full objective for learning anchors in hindsight from the episodic memory. 
%
We note that this approximation of future by replaying past data is effective for many continual learning benchmarks as evidenced in our experiments (Table~\ref{table:oracle_access}).
%

This completes the description of our proposed algorithm for continual learning, which combines experience replay with anchors learned in hindsight.
%
We call our approach Hindsight Anchor Learning (\ours{}) and summarize the entire learning process as follows:
%\vspace*{0.2cm}
\begin{mdframed}[backgroundcolor=yellow!8]
\vspace*{0.2cm}
\textbf{Hindsight Anchor Learning (\ours{})}
\begin{itemize}
    \item Initialize $\theta \sim P(\theta)$ and $\{e_t \sim P(e)\}_{t=1}^T$ from normal distributions $P(\theta)$ and $P(e)$.
    \item Initialize $\mathcal{M} = \{\}$
    \item For each task $t = 1, \ldots, T$:
    \begin{itemize}
        \item Initialize $\phi_t = 0$
        \item For each minibatch $\mathcal{B}$ from task $t$:
        \begin{itemize}
            \item Sample $\mathcal{B}_\mathcal{M}$ from $\mathcal{M}$
            \item Update $\theta$ using \eqref{eq:main_update}
            \item Update $\phi_t$ using \eqref{eq:mean_embedding}
            \item Update $\mathcal{M}$ by adding $\mathcal{B}$ in a first-in first-out (FIFO) ring buffer  
        \end{itemize}
        \item Fine-tune on $\mathcal{M}$ to obtain $\theta_{\mathcal{M}}$ 
        \item Build $e_t$ using \eqref{eq:anchors_2} $k$ times
        \item Discard $\phi_t$
    \end{itemize}
    \item Return $\theta$.
\end{itemize}
%\vspace*{0.2cm}
\end{mdframed}

==> impact.tex <==
\section{Broader Impact} \label{sec:impact}

%This section is not applicable to our work as we focus on a core ML method.

Continuous learning methods like the one we propose allow models to learn on new data in a more agile way, preserving old knowledge without requiring constant retraining. This allows machine learning systems to react and adapt much faster to changes in data distribution while still being performant on old tasks.
Continuous learning, however, hinges on the assumption that not forgetting is a desirable property. 
In some scenarios, partially forgetting old data may be acceptable or even preferable, for example if older data was more biased (in any sense) than more recent data. Practitioners should be aware of this fact and use continuous learning approaches only when suitable.
